SDC Resilient Error-bounded Lossy Compressor

Lossy compression is one of the most important strategies to resolve the big science data issue, however, little work was done to make it resilient against silent data corruptions (SDC). In fact, SDC is becoming non-negligible because of exa-scale computing demand on complex scientific simulations with vast volume of data being produced or in some particular instruments/devices (such as interplanetary space probe) that need to transfer large amount of data in an error-prone environment. In this paper, we propose an SDC resilient error-bounded lossy compressor upon the SZ compression framework. Specifically, we adopt a new independent-block-wise model that decomposes the entire dataset into many independent sub-blocks to compress. Then, we design and implement a series of error detection/correction strategies based on SZ. We are the first to extend algorithm-based fault tolerance (ABFT) to lossy compression. Our proposed solution incurs negligible execution overhead without soft errors. It keeps the correctness of decompressed data still bounded within user's requirement with a very limited degradation of compression ratios upon soft errors.

==> tex/decmp_ana.tex <==
\section{Analysis of Decompression}
\label{sec:decompanalysis}

The above analysis focus on the soft errors in the compression procedure of SZ. Algorithm~\ref{alg: ft sz} will make sure that the compression procedure of SZ is soft error resilient under our error model. To make SZ soft error resilient, we need to analyze the fault tolerance of decompression procedure in SZ too. Recall that the basic steps in decompression of SZ is: decompressing the byte file using lossless decompression, decoding by Huffman tree and then reversing the Lorenzo or regression procedure in compression. 

\subsection{computation error}

\subsubsection{Two possible solutions without duplication}
Without duplicating all the instructions in decompression, we come up with two solutions. The first one is a straightforward application of ABFT. We will calculate the sum of all decompressed data for each block in compression and store the sum to output file. Then we will verify if the sum of each block of decompressed data in decompression is identical to the one done in compression. If this is not identical, we can simply rerun that block of decompression. The second solution will make use of the fact that the coefficients are already existing when we do decompression and they have equations with the sum of each block of data as following \textcolor{red}{cite}:
\begin{equation}
    sum = n_1n_2n_3[\beta_0 + (\frac{n_1-1}{2}\beta_1 + \frac{n_2-1}{2}\beta_2 + \frac{n_3-1}{2}\beta_3)]
\label{equa: sum and coe}
\end{equation}
In equation~\ref{equa: sum and coe}, $n_i$ is the dimension size of the $i$th dimension of the dataset (\textcolor{red}{block size?}); $\beta_i$ are the coefficients for each block of dataset. According to equation~\ref{equa: sum and coe}, we could get the sum of original input data from the coefficients.

\subsubsection{Comparison of the two solutions} In terms of performance overhead to the original SZ, the second solution is better since it does not require to store the checksums of the decompressed data which has both lower compression ratio overhead and lower compression rate overhead. However, in terms of error detection accuracy, the first solution is better than the second one. The first reason is that the first solution checksumming the decompressed data in compression directly while the second solution restore the sum of original input data. As we know, SZ is a lossy compression which means there will be a difference between original and decompressed data. This means the second solution will only detect the errors which lead to significant deviation. Specifically, the difference can be as large as $|ne|$ where $n$ is the number of data in each block and $e$ is the error bound. The second reason is that the coefficients ($\beta_i$) are also not accurate since they were also compressed by lossy methods. So according to equation~\ref{equa: sum and coe}, the inaccuracy in coefficients will be magnified by at least $n_1n_2n_3$. Those two reasons will decrease the detection accuracy or error coverage of the second solution. So in this paper, we use the first solution to detect memory error or computation error in decompression. Again, we treat the floating point numbers as integers and calculate the checksum to avoid round off error. Since we need to store a checksum (64-bit integer) for each block of data, this may introduce a overhead to the compression ratio. To mitigate the compression ratio overhead, we can use lossless compression to compress the checksums for decompressed data in compression.


\subsection{memory error}
%Since the dominant part is the reverse procedure of Lorenzo or regression, the decompressed data may be corrupted before the whole decompression procedure finishes. So we decide to introduce the checksums for the decompressed data to be resilient to the memory error. We detail the fault tolerant decompression of SZ in Algorithm~\ref{alg: ft sz decmpr}.
The first solution for detecting computation errors also works for detecting memory error since no matter which kind of error it is, the checksum directly verifies if the decompressed data is the same with the one in compression and both computation error and memory error will lead to incorrect decompressed data. We detail the fault tolerant decompression of SZ in Algorithm~\ref{alg: ft sz decmpr}.


\begin{algorithm}
\caption{\textsc{Soft Error Resilient SZ Decompression}} \label{alg: ft sz decmpr}
\renewcommand{\algorithmiccomment}[1]{/*#1*/}
\footnotesize
\textbf{Input}: The SZ compressed file in byte (cmp\_data) \textcolor{blue}{and compressed $sum$ for blocked decompressed data (cmp\_sum)}. 

\textbf{Output}: The decompressed data which has bounded error with the original data.

\begin{algorithmic}[1]

\STATE lossless decompress cmp\_data
\STATE $q\_bin[] \gets$ decode using Huffman tree
\STATE $sum[] \gets $ lossless decompress cmp\_sum 
\FOR {each block of $q\_bin[]$}
\IF {it was compressed by Lorenzo}
\STATE $dec\_data[] \gets $ Lorenzo decompression
\ELSE
\STATE $dec\_data[] \gets $ regression decompression
\ENDIF
\STATE \textcolor{blue}{ calculate current $cur\_sum$ for this block of $dec\_data[]$}
\IF {\textcolor{blue}{ $cur\_sum != sum[i]$}}
\STATE \textcolor{blue}{ re-execute decompression for block $i$}
\ENDIF
\ENDFOR

\STATE \textcolor{blue}{detect memory error again after $dec\_data[]$ is complete}


\end{algorithmic}

\end{algorithm}


==> tex/extension2para.tex <==
\section{Extension to Parallel Sorting}
\label{section: extension to parallel}
\vspace{-.1cm}

%\textcolor{green}
{Our fault-tolerant strategy also applies to parallel sorting algorithms based on $introsort$. To the best of our knowledge, HykSort\cite{hyksort} is the most well-known parallel sorting.}
%\vspace{-0.6cm}
\subsection{HykSort}
\vspace{-.1cm}
%\textcolor{green}
{Given a global array, the size of which far exceeds the memory limit of one computing node, HykSort performs parallel sorting using introsort, following the procedure below: 
\begin{enumerate}
\item Each process loads a part of the array; that is, the global array is partitioned into multiple local arrays, each local array kept by one process. 
\item Each process sorts the allotted local array using introsort. 
\item Each process partitions the assigned local array into $k$ partitions based on $k-1$ global pivots. 
\item Processes exchange partitions, ensuring that processes with lower ranks receive partitions with lesser elements and processes with higher ranks receive partitions with greater elements.
\item {{Each process merges the $k$ sorted partitions it received.}}
\item The sorting completes if the following requirements are met: (a) the local array of each process is well-sorted, and (b) $e_i < e_j$, where $e_i$ denotes any element from process $i$, $e_j$ denotes any element from process $j$, and $0 \le i < j < p$ where $p$ is the total number of processes; otherwise, the sorting goes back to Step 3.
\vspace{-.2cm}
\end{enumerate}}

%\vspace{-0.05in}
\subsection{Fault-Tolerant HykSort}
\vspace{-.1cm}

\subsubsection{{Protection for Comparisons}}

%\textcolor{green}
{\textit{90\% coverage.} Our fault-tolerant introsort is constructed to be naturally contained in the GNU Standard C++ Library. Without any code changes to HykSort, 90\% of comparisons of HykSort can be achieved by linking to the library as before. We denote the global array length, the number of processes, and the number of partitions  respectively as $N$, $p$ and $k$. Local array length is given by $n=\frac{N}{p}$. The number of comparisons in local sorting, partitioning, and merging are respectively $n \log n$ (lower bound), $k \log {n}$ and $n \frac{\log p}{\log k} $ ~\cite{hyksort}. Since our fault-tolerant introsort only protects local sorting, the \textit{error coverage} is the ratio of the number of comparisons in introsort to the total number of comparisons in HykSort:}
\vspace{-.3cm}
\begingroup\makeatletter\def\f@size{8}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}%
\begin{equation}
Cov = \frac{n\log n}{n \log n + k \log n + n \frac{\log p}{\log k}}= \frac{1}{1+\frac{k}{n}+\frac{\log p}{\log n \log k}}
\label{equ:coverage}
\vspace{-.1cm}
\end{equation}\endgroup
%\textcolor{green}
{HykSort uses $k = 128$ by design. The only variables here are $n$ and $p$. We calculate the lower bound of error coverage according to standard experimental settings \cite{hyksort}.
In weak scaling, the setting with the lowest coverage is: $n = 2^{25}$, $p = 2^{18} = 262,144$. Incorporating these numbers into the formula, we get $90.7\%$ coverage. In strong scaling, $N = 2^{38}$ and $p = 2^{18}$ yields the lowest coverage at $88.6\%$. These calculations show our fault-tolerant introsort protects about $90\%$ of the comparisons in Hyksort.}

%\textcolor{green}
{\textit{100\% coverage.}  {To protect the comparisons outside local sort{ing}, we propose {the use of} TMR for the negligible amount {($k \log n$) of} comparisons in partitioning {in} step 3; we adapt Ravikumar's analysis\cite{FT merge} to protect step 5 of HykSort, which is the \emph{k-sorted-merge}. We present the following corollary:}}

{Given $k$ sorted subarrays, {the subarrays can be} merged into a single sorted array with at most $e$ comparison errors. The runs of the output will be at most $e+1$.}

\textit{Proof:} {Ravikumar proves that if there are $e$ comparison errors {in a} standard mergesort, the output array will have {a runs of} at most $e+1$\cite{FT merge}. Suppose all $e$ comparison errors happen after $k$ sorted subarrays are finished: the later procedure will be exactly a \emph{k-sorted-merge}, and the corollary holds true.\qed}

{Based on this analysis, a similar error correction technique for heapsort output, \emph{e-sorted-merge}, can be applied to the \emph{k-sorted-merge}. Obviously, if $e>k-1$, the correction technique {complexity} ($n\log (e+1)$) is reduced to the original problem complexity ($n\log k$). {We recommend taking advantage of our prior knowledge of the error rate, $e <\log n$,} and using \emph{e-sorted-merge} to protect \emph{k-sorted-merge} if $e<k-1$. If $e>k-1$, TMR may be used for \emph{k-sorted-merge}. }
%\textcolor{red}{I don't like the blue sentence, it looks like we couldn't be bothered to analyze this potential overhead. We are better off just stating how we will obtain 100\% coverage without commenting on overhead; or we could cite someone else's findings for TMR protection of these 10\% comparisons (if they exist)}\textcolor{blue}{The potential overhead is expected to be trivial considering the comparisons outside local sort (introsort) only accounts for about 10\%.}} \textcolor{yellow}{will see how to handle this later...}

\subsubsection{Protection for Memory}
\label{sec:hyksort mem}
%\textcolor{green}
{To tolerate memory errors in Hyksort, we introduce Xor-based re-execution ($XR$) to Hyksort as following:
\begin{itemize}
\item Apply $XR$ to local sorting (introsort).
\item When all local sorts are complete, reduce the local Xors across all processes to get a global Xor.
\item When global sorting is complete, each process calculates a local Xor and reduce to obtain another global Xor.
\item If the two global Xors vary, re-execute Hyksort.
\end{itemize}
The logic is clear: $XR$ applied to introsort protects the memory errors in local sorting, and global Xors guard against memory errors outside local sorting.}

==> tex/mem_err_ana.tex <==
\section{Analysis of Memory Error}
\subsection{Memory error in input data}
The input data takes $n$ units of memory. So we think a memory error may happen to the input data. We notice that the input data is used in the following steps: computing the regression coefficients; computations in prediction including calculating the difference between predicted data and original data and handling unpredictable data; and estimating the error of both regression based compression and Lorenzo prediction based compression. Now we analyze if the input data needs to be protected in each of the step. If yes, how we can protect the memory using ABFT.

\subsubsection{Computation of regression coefficients} In this procedure, we need to calculate the checksums by Equation (\ref{equa:sum}) and Equation (\ref{equa: isum}) so that in the future when the input data is used again, we can verify if the input data is corrupted or not. We have to assume that there is no memory error before the checksums are calculated because the checksums are only effective to detect and correct memory errors that happen after checksums are calculated. In practice, since the input data are used block by block, the checksums are also calculated block by block. I. e., each block of input data has their own checksums which can be used to detect and correct memory error in that block.

\subsubsection{Prediction} In prediction, we need to calculate the difference between predicted data and original data. We also need to access the original data if we find the data is unpredictable. Thus we need to confirm that before the input data is used, it was not corrupted by memory error. It is obvious that if the corrupted input data was used in prediction, the decompressed data will be within the error bound of the corrupted data while not the genuine data. \textcolor{red}{for this part, we may be able to tolerate some flips that are negligible: see the value change can let us know the bit flip position.} To verify that the input data was not corrupted by memory error before it is used, we need to first calculate the sum, $sum1'$, of the block of input data and see if this matches with what we calculated before. If it is a match, we believe there was not memory error. If not, we need to calculate the $isum1'$ according to Equation (\ref{equa:isum}) and correct the corrupted data using the ABFT as we discussed in Section~\ref{sec:abft}.

\subsubsection{Estimating Lorenzo and regression errors} For each block of input data, to determine which strategy compress better, SZ estimates the compression error by sampling a portion of input data. It will then choose the one that has smaller errors to compress that block. To estimate Lorenzo's error without compressing all the data in that block, SZ uses original data while not decompressed data to estimate the error. So the original input data is used in this part of calculation. The corrupted value will make the estimation of compression error for Lorenzo varies from the correct estimation. However, since the estimation error will only impact which strategy (Lorenzo or regression) to use, it will only impact the compression ratio while not the correctness of compression or decompression. This means we do not have to check if the checksums vary or not.

\subsection{Memory error in regression coefficients} 

\subsection{Memory error in type array} In SZ, the type array is used to record the quantization bins. The element in the type array is a positive integer if the data it records is predictable; otherwise, the element will be 0. When each data is predicted in compression, we will get its element in the type array. Since this is one of the execution time dominant part, we need to protect the type array from memory errors. Specifically, we accumulate the two checksums right after each data inside a single block is processed. Then when we want to do Huffman encoding, we are able to check if each block of type array still has the same checksum. If not, we will be able to correct the corrupted value.

\subsection{Memory error in decompressed data} The decompressed data will be calculated both in compression and decompression. We will only calculate $sum$ but not $isum$ for decompressed data in compression. With this $sum$, we are able to detect both computation error and memory error when decompressed data is computed in decompression. Notice that the decompressed data in compression will not be held for a long time since it will only be used for predicting neighbor data. We will detail the analysis of the $sum$ for detecting decompression errors in the next section (Section~\ref{section: decomp analysis}). 

\subsection{Handling round off error} Obviously, the input data and the regression coefficients are both floating point numbers. That will make our calculations of checksums vary even when there is no memory error. The round off error will let our memory error detection and correction not accurate. To avoid this issue, we propose to treat the 32-bit floating point numbers as 32-bit unsigned integers and then we calculate checksums based on these integers. This trick will let us be able to achieve 100\% accurate detection and correction under the error model that there is at most one soft error during one single SZ execution. 

\subsection{Wrap it up} In the above 2 Sections, we have analyzed the impact of computation error and memory error. Now, we will detail the whole fault tolerant SZ compression algorithm in Algorithm~\ref{alg: ft sz cmpr}.



%\begin{comment}

\begin{algorithm}
\caption{\textsc{Soft Error Resilient SZ Compression}} \label{alg: ft sz cmpr}
\renewcommand{\algorithmiccomment}[1]{/*#1*/}
\footnotesize
\textbf{Input}: original input data (denote by $ori[]$), user defined error bound (denoted by $e$).

\textbf{Output}: compressed data in byte \textcolor{blue}{and compressed $sum$ of blocked decompressed data}

\begin{algorithmic}[1]

\FOR {each block (block $i$) of in the input data}

\STATE compute the regression coefficients
\STATE \textcolor{blue}{ calculate $sum[i]$ on input data by equation~\ref{equa: sum}}
\STATE \textcolor{blue}{ calculate $isum[i]$ on input data by equation~\ref{equa: isum}}
\ENDFOR


\FOR {each block of input data}
\STATE \textcolor{blue}{ memory error detection and correction for this block}
\STATE sample and estimate $E_{reg}$ and $E_{lor}$
\COMMENT{$E_{reg}$ is for regression error; $E_{lor}$ is for Lorenzo error}

\IF {regression error $>$ Lorenzo error}
\FOR {each data point, $ori$, in each data block }
\STATE $pred' \gets f(pred'_{pre})$ \COMMENT{\textcolor{blue}{ duplication}}
\STATE $diff \gets ori - pred'$
\STATE $q\_bin \gets quant(diff, e)$ \COMMENT{calcualte quantization bin based on $diff,e$}
\IF {$q\_bin$ is not in the acceptable bin range}
\STATE compress $ori$ as unpredictable
\ELSE
\STATE keep $q\_bin[]$ in memory
\STATE \textcolor{blue}{ accumulate $sum$, $isum$ for $q\_bin[]$}
\STATE $dcmp \gets dec(q\_bin, pred') $ \COMMENT{\textcolor{blue}{ duplication}}
\IF { $|ori - dcmp| > e$}
\STATE compress $ori$ as unpredictable
\ENDIF
\STATE \textcolor{blue}{accumulate only $sum$ for $dcmp$}
\ENDIF

\ENDFOR
\ENDIF
\ENDFOR

\FOR {each block of $q\_bin[]$}
\STATE \textcolor{blue}{memory error detection and correction}
\STATE histogram $q\_bin[]$
\ENDFOR

\STATE construct Huffman tree
\FOR {each block of $q\_bin[]$}
\STATE \textcolor{blue}{memory error detection and correction}
\STATE encode $q\_bin[]$ by Huffman tree
\ENDFOR
\STATE compress encoded $q\_bin$ by lossless method
\STATE write compressed $q\_bin$ and unpredictable data to byte file
\STATE \textcolor{blue}{ compress all $sum$ for each block of $dcmp$ by lossless method and write to file}
\end{algorithmic}

\end{algorithm}
%\end{comment}

==> tex/random_access.tex <==
\section{Achieving Blockwise Dependency}
Recall that though SZ 2.0 is implemented in a blockwise way, to maximize the compression ratio, there is still data dependency between two neighbor blocks if the blocks were using Lorenzo predictor. However, in terms of resilience, the data dependency between neighbor blocks can propagate a single memory error or computation error till the end of the whole data array. Now we discuss how to eliminate the dependency between blocks which will always limit the error propagation inside its own block while other blocks will not be affected.

Another benefit that we can gain from eliminating the data dependency between neighbor blocks is we can decompress any given range of blocks of data. This is very meaningful when the user just want to decompress part of the whole data. We thus call our improved SZ 2.0 as randomly accessible SZ 2.0. Also, eliminating the dependency between blocks will make the parallelism of SZ much easier.

The main difference of the designs between the original SZ 2.0 and our proposed randomly accessible SZ 2.0 is that we now treat each block of data as an individual data block and apply our SZ compression techniques inside each individual block. Another difference is for the goal of randomly accessible decompression. We record the compressed size of each block of data after we finish compression for that block. This will be a must since without this information, given a desired range of data to be decompressed, we do not know its corresponding start and end offset in the decompressed file.


